A Position Allocation Approach to the Scheduling of Battery-Electric Bus Charging

Robust charging schedules in a growing market of battery electric bus (BEB) fleets are a critical component to successful adoption. In this paper, a BEB charging scheduling framework that considers spatiotemporal schedule constraints, route schedules, fast and slow charging, and battery dynamics is modeled as a mixed integer linear program (MILP). The MILP is modeled after the Berth Allocation Problem (BAP) in a modified form known as the Position Allocation Problem (PAP). Linear battery dynamics are included to model the charging of buses while at the station. To model the BEB discharges over their respective routes, it is assumed each BEB has an average kWh charge loss while on route. The optimization coordinates BEB charging to ensure that each vehicle remains above a specified state-of-charge (SOC). The model also minimizes the total number of chargers utilized and prioritizes slow charging for battery health. The model validity is demonstrated with a set of routes sampled from the Utah Transit Authority (UTA) for \A buses and \N visits to the charging station. The model is also compared to a heuristic algorithm based on charge thresholds referred to as the Qin-Modified method. The results presented show that the slow chargers are more readily selected and the charging and spatiotemporal constraints are met while considering the battery dynamics and minimizing both the charger count and consumption cost.

==> org-doc-scripts/build-pdf <==
#!/bin/sh

#===============================================================================
# DESCRIPTION
#
# This script builds a LaTeX file using `latexmk'.
#===============================================================================

# Build the document
latexmk -f -interaction=nonstopmode \
           -pdf -pdflatex="pdflatex --shell-escape %O %S" \
           -bibtex ${1}.tex

# Rename the document to TARGET
mv ${1}.pdf ${2}

